TempRetriever: Fusion-based Temporal Dense Passage Retrieval for Time-Sensitive Questions

Temporal awareness is crucial in many information retrieval tasks, particularly in scenarios where the relevance of documents depends on their alignment with the query's temporal context. Traditional approaches such as BM25 and Dense Passage Retrieval (DPR) focus on lexical or semantic similarity but tend to neglect the temporal alignment between queries and documents, which is essential for time-sensitive tasks like temporal question answering (TQA). We propose TempRetriever, a novel extension of DPR that explicitly incorporates temporal information by embedding both the query date and document timestamp into the retrieval process. This allows retrieving passages that are not only contextually relevant but also aligned with the temporal intent of queries. We evaluate TempRetriever on two large-scale datasets ArchivalQA and ChroniclingAmericaQA demonstrating its superiority over baseline retrieval models across multiple metrics. TempRetriever achieves a 6.63\% improvement in Top-1 retrieval accuracy and a 3.79\% improvement in NDCG@10 compared to the standard DPR on ArchivalQA. Similarly, for ChroniclingAmericaQA, TempRetriever exhibits a 9.56\% improvement in Top-1 retrieval accuracy and a 4.68\% improvement in NDCG@10. We also propose a novel, time-based negative sampling strategy which further enhances retrieval performance by addressing temporal misalignment during training. Our results underline the importance of temporal aspects in dense retrieval systems and establish a new benchmark for time-aware passage retrieval.

==> tables/_backup_main_result.tex <==
\begin{comment}
\begin{table}[ht]
\centering
\resizebox{1\textwidth}{!}{  % Resize the table to fit the page width

\begin{tabular}{l|l|cccccc|cccccc} %|cccccc
\hline
\multirow{2}{*}{\textbf{Retriever}}& \multirow{2}{*}{\textbf{Mode}}  & \multicolumn{6}{c|}{\textbf{Val }} & \multicolumn{6}{c}{\textbf{ Test }}  \\ %& \multicolumn{6}{c}{\textbf{WEBQ}}
 & &Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100 & Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100  \\ %& Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100

\midrule


\multirow{4}{*}{\textbf{ArchivalQA}} & NoDate 
  & $63.09 \pm 0.76$  & $82.42 \pm 0.29$  & $87.47 \pm 0.11$  & $90.97 \pm 0.15$  & $94.40 \pm 0.21$  & $96.14 \pm 0.03$
  & $62.98 \pm 0.55$  & $82.50 \pm 0.33$  & $87.17 \pm 0.45$  & $90.97 \pm 0.27$  & $94.64 \pm 0.23$  & $96.15 \pm 0.16$   \\
  
  & DateAsToken   
  & $63.51 \pm 0.32$  & $83.41 \pm 0.28$  & $88.52 \pm 0.08$  & $91.97 \pm 0.08$  & $94.92 \pm 0.05$  & $96.52 \pm 0.02$  
  & $63.44 \pm 0.29$  & $83.23 \pm 0.05$  & $88.35 \pm 0.10$  & $91.72 \pm 0.03$  & $94.94 \pm 0.23$  & $96.72 \pm 0.08$\\

  & DateAsTag 
  & $57.94 \pm 0.71$  & $78.78 \pm 0.61$  & $84.28 \pm 0.41$  & $88.48 \pm 0.48$  & $92.43 \pm 0.26$  & $94.64 \pm 0.13$ 
  & $58.37 \pm 0.70$  & $78.43 \pm 0.84$  & $83.93 \pm 0.45$  & $88.21 \pm 0.41$  & $92.77 \pm 0.25$  & $94.93 \pm 0.10$  \\
  
  & DateEmbedding   
  & $64.80 \pm 0.34$  & $84.95 \pm 0.32$  & $89.35 \pm 0.09$  & $92.63 \pm 0.06$  & $95.41 \pm 0.12$  & $96.73 \pm 0.03$  
    & $65.10 \pm 0.86$  & $84.78 \pm 0.46$  & $89.42 \pm 0.36$  & $92.84 \pm 0.35$  & $95.77 \pm 0.23$  & $97.13 \pm 0.13$ \\
\bottomrule

\multirow{4}{*}{\textbf{ChroniclingQA}} & NoDate 
  & $44.97 \pm 0.24$  & $61.14 \pm 0.16$  & $67.86 \pm 0.16$  & $73.32 \pm 0.21$  & $79.12 \pm 0.10$  & $83.53 \pm 0.15$ 
    & $45.70 \pm 0.46$  & $60.47 \pm 0.25$  & $67.40 \pm 0.14$  & $72.20 \pm 0.18$  & $78.69 \pm 0.13$  & $82.26 \pm 0.09$ \\
  
  & DateAsToken 
  & $44.81 \pm 0.04$  & $61.28 \pm 0.28$  & $67.62 \pm 0.16$  & $73.60 \pm 0.13$  & $79.12 \pm 0.25$  & $83.17 \pm 0.07$
    & $45.81 \pm 0.09$  & $60.79 \pm 0.19$  & $66.58 \pm 0.20$  & $72.09 \pm 0.15$  & $78.82 \pm 0.07$  & $82.10 \pm 0.22$  \\
  
  & DateAsTag 
  & $45.00 \pm 0.17$  & $61.48 \pm 0.31$  & $67.62 \pm 0.19$  & $72.97 \pm 0.07$  & $79.14 \pm 0.18$  & $82.99 \pm 0.18$
    & $45.75 \pm 0.48$  & $60.77 \pm 0.49$  & $66.77 \pm 0.22$  & $72.44 \pm 0.32$  & $78.72 \pm 0.18$  & $81.89 \pm 0.21$  \\
  
  & DateEmbedding  
  & $50.22 \pm 0.19$  & $64.88 \pm 0.23$  & $71.16 \pm 0.30$  & $77.90 \pm 0.21$  & $83.05 \pm 0.11$  & $86.22 \pm 0.29$
    & $50.10 \pm 0.10$  & $66.01 \pm 0.17$  & $71.85 \pm 0.39$  & $77.19 \pm 0.11$  & $82.81 \pm 0.25$  & $86.52 \pm 0.10$  \\
\bottomrule
\end{tabular}}
\caption{Top-\{1,5,10,20,50,100\} retrieval accuracy for ArchivalQA and ChroniclingQA explicit datasets, evaluated on both validation and test sets. The results measure the percentage of top retrieved passages that contain the correct answer across different temporal retrieval models, including the baseline Vanilla, Date as Token, Date as Tag, and Date Embedding approaches.}
\end{table}
\end{comment}

\begin{table}[ht]
\centering
\setlength\tabcolsep{5pt}
\resizebox{1\textwidth}{!}{  % Resize the table to fit the page width

\begin{tabular}{l|l|cccccc} %|cccccc
\hline
\multirow{2}{*}{\textbf{Dataset}}& \multirow{2}{*}{\textbf{Mode}}  & \multicolumn{6}{c}{\textbf{Validation Results}}   \\ %& \multicolumn{6}{c}{\textbf{WEBQ}}
 & &Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100 \\ %& Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100

\midrule


\multirow{4}{*}{\textbf{ArchivalQA}} & NoDate 
  & $63.09_{\pm 0.76}$  & $82.42_{\pm 0.29}$  & $87.47_{\pm 0.11}$  & $90.97_{\pm 0.15}$  & $94.40_{\pm 0.21}$  & $96.14_{\pm 0.03}$\\
  
  & DateAsToken   
  & $63.51_{\pm 0.32}$  & $83.41_{\pm 0.28}$  & $88.52_{\pm 0.08}$  & $91.97_{\pm 0.08}$  & $94.92_{\pm 0.05}$  & $96.52_{\pm 0.02}$ \\ 


  & DateAsTag 
  & $57.94_{\pm 0.71}$  & $78.78_{\pm 0.61}$  & $84.28_{\pm 0.41}$  & $88.48_{\pm 0.48}$  & $92.43_{\pm 0.26}$  & $94.64_{\pm 0.13}$ \\
 
  
  & TempDPR  
  & \textbf{$64.80_{\pm 0.34}$}  & \textbf{$84.95_{\pm 0.32}$}  & \textbf{$89.35_{\pm 0.09}$}  & \textbf{$92.63_{ \pm 0.06}$}  & \textbf{$95.41_{\pm 0.12}$}  & \textbf{$96.73_{\pm 0.03}$}  \\
  
\midrule

\multirow{4}{*}{\textbf{ChroniclingQA}} & NoDate 
  & $44.97_{\pm 0.24}$  & $61.14_{\pm 0.16}$  & $67.86_{\pm 0.16}$  & $73.32_{\pm 0.21}$  & $79.12_{\pm 0.10}$  & $83.53_{\pm 0.15}$ \\
  
  & DateAsToken 
  & $44.81_{\pm 0.04}$  & $61.28_{\pm 0.28}$  & $67.62_{\pm 0.16}$  & $73.60_{\pm 0.13}$  & $79.12_{\pm 0.25}$  & $83.17_{\pm 0.07}$\\
  
  & DateAsTag 
  & $45.00_{\pm 0.17}$  & $61.48_{\pm 0.31}$  & $67.62_{\pm 0.19}$  & $72.97_{ \pm 0.07}$  & $79.14_{ \pm 0.18}$  & $82.99_{ \pm 0.18}$\\
  
  & TempDPR  
  & $50.22_{\pm 0.19}$  & $64.88_{\pm 0.23}$  & $71.16_{\pm 0.30}$  & $77.90_{ \pm 0.21}$  & $83.05_{\pm 0.11}$  & $86.22_{\pm 0.29}$\\
\bottomrule
\end{tabular}}

\resizebox{1\textwidth}{!}{  % Resize the table to fit the page width

\begin{tabular}{l|l|cccccc} %|cccccc
\hline
\multirow{2}{*}{\textbf{Dataset}}& \multirow{2}{*}{\textbf{Mode}}  & \multicolumn{6}{c}{\textbf{Test Results }}  \\ %& \multicolumn{6}{c}{\textbf{WEBQ}}
 & &Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100  \\ %& Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100
\midrule

\multirow{4}{*}{\textbf{ArchivalQA}} & NoDate 

  & $62.98_{ \pm 0.55}$  & $82.50_{ \pm 0.33}$  & $87.17_{ \pm 0.45}$  & $90.97_{ \pm 0.27}$  & $94.64_{ \pm 0.23}$  & $96.15_{ \pm 0.16}$   \\
  
  & DateAsToken   
  
  & $63.44_{ \pm 0.29}$  & $83.23_{ \pm 0.05}$  & $88.35_{ \pm 0.10}$  & $91.72_{ \pm 0.03}$  & $94.94_{ \pm 0.23}$  & $96.72_{ \pm 0.08}$\\

  & DateAsTag 

  & $58.37_{ \pm 0.70}$  & $78.43_{ \pm 0.84}$  & $83.93_{ \pm 0.45}$  & $88.21_{ \pm 0.41}$  & $92.77_{ \pm 0.25}$  & $94.93_{ \pm 0.10}$  \\
  
  & TempDPR   
 
    & $65.10_{ \pm 0.86}$  & $84.78_{ \pm 0.46}$  & $89.42_{ \pm 0.36}$  & $92.84_{ \pm 0.35}$  & $95.77 _{\pm 0.23}$  & $97.13_{ \pm 0.13}$ \\
\midrule

\multirow{4}{*}{\textbf{ChroniclingQA}} & NoDate 

    & $45.70_{ \pm 0.46}$  & $60.47_{ \pm 0.25}$  & $67.40_{ \pm 0.14}$  & $72.20_{ \pm 0.18}$  & $78.69_{ \pm 0.13}$  & $82.26_{ \pm 0.09}$ \\
  
  & DateAsToken 

    & $45.81_{ \pm 0.09}$  & $60.79_{ \pm 0.19}$  & $66.58_{ \pm 0.20}$  & $72.09_{ \pm 0.15}$  & $78.82_{ \pm 0.07}$  & $82.10_{ \pm 0.22}$  \\
  
  & DateAsTag 

    & $45.75_{ \pm 0.48}$  & $60.77_{ \pm 0.49}$  & $66.77_{ \pm 0.22}$  & $72.44_{ \pm 0.32}$  & $78.72_{ \pm 0.18}$  & $81.89_{ \pm 0.21}$  \\
  
  & TempDPR  
    & $50.10_{ \pm 0.10}$  & $66.01_{ \pm 0.17}$  & $71.85_{ \pm 0.39}$  & $77.19_{ \pm 0.11}$  & $82.81_{ \pm 0.25}$  & $86.52_{ \pm 0.10}$  \\
\bottomrule
\end{tabular}}
\caption{Top-\{1,5,10,20,50,100\} retrieval accuracy for ArchivalQA and ChroniclingQA explicit datasets, evaluated on both validation and test sets. The results measure the percentage of top retrieved passages that contain the correct answer across different temporal retrieval models, including the baseline Vanilla, Date as Token, Date as Tag, and Date Embedding approaches.}
\label{tab:top-explicit_dataset}
\end{table}


\begin{comment}
    
\begin{table}[ht]
\centering
\resizebox{1\textwidth}{!}{  % Resize the table to fit the page width

\begin{tabular}{l|l|cccccc|cccccc} %|cccccc
\hline
\multirow{2}{*}{\textbf{Retriever}}& \multirow{2}{*}{\textbf{Mode}}  & \multicolumn{6}{c|}{\textbf{Val }} & \multicolumn{6}{c}{\textbf{Test}}  \\ %& \multicolumn{6}{c}{\textbf{WEBQ}}
 & &1 & 5 & 10 & 20 & 50 & 100 & 1 & 5 & 10 & 20 & 50 & 100  \\ %& Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100

\midrule
\multirow{4}{*}{\textbf{ArchivalQA}} & NoDate  & 48.59 & 59.20 & 61.25 & 62.49 & 63.69 & 64.31 & 48.66& 59.38 & 61.25 & 62.61 & 63.84 &  64.43 \\

 & DateAsToken & 47.61& 58.48 & 60.71  &  62.17 &  63.35 & 63.95 & 47.89 & 58.64 & 60.76 & 62.17&63.42 &  64.05\\

 & DateAsTag & 42.06 &  52.49 & 54.71 &  56.26&57.62  &58.31  &43.12  & 53.27 & 55.47 &  56.96&58.32 &  59.04  \\
 
 & DateEmbedding & 50.12 & 61.25 & 63.22 & 64.55 & 65.73 & 66.24 & 50.62 &61.49 & 63.53 &64.91 & 66.05 & 66.54 \\
%MSS-DPR         &  &  &  & &  &  & &  &   & &  &  \\

\midrule
\multirow{4}{*}{\textbf{ChroniclingQA}} & NoDate & 39.72 & 47.06 & 48.35 & 49.36 & 50.38 & 50.86 & 41.2 & 47.54 & 48.87 & 49.74 & 50.68 & 50.97 \\
 & DateAsToken & 39.72 & 47.06 & 48.35 & 49.36 & 50.38 & 50.86 & 41.2 & 47.54 & 48.87 & 49.74 & 50.68 & 50.97 \\
 & DateAsTag & 40.21 & 47.00 & 48.24 & 49.16 & 50.31 & 50.82 & 41.2 & 47.03 & 48.41 & 49.55 & 50.39 & 50.93 \\
 & DateEmbedding & 44.35 & 51.79 & 53.03 & 54.23 & 55.24 & 55.75 & 44.83 & 51.44 & 52.85 & 53.88 & 55.01 & 55.33 \\

\bottomrule
\end{tabular}}
\caption{Results (NDCG@\{1,5,10,20,50,100\}) for the ArchivalQA and ChroniclingQA explicit datasets across validation and test sets.}
\end{table}


\begin{table}[ht]
\centering
\resizebox{1\textwidth}{!}{  % Resize the table to fit the page width

\begin{tabular}{l|l|cccccc|cccccc} %|cccccc
\hline
\multirow{2}{*}{\textbf{Retriever}}& \multirow{2}{*}{\textbf{Mode}}  & \multicolumn{6}{c|}{\textbf{Val }} & \multicolumn{6}{c}{\textbf{Test}}  \\ %& \multicolumn{6}{c}{\textbf{WEBQ}}
 & &1 & 5 & 10 & 20 & 50 & 100 & 1 & 5 & 10 & 20 & 50 & 100  \\ %& Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100

\midrule
\multirow{4}{*}{\textbf{ArchivalQA}} & NoDate & 48.56 & 56.17 & 57.02 &57.36  & 57.56 & 57.62 & 48.64 & 56.33 & 57.12 &57.49 & 57.69&  57.74\\

 & DateAsToken & 47.58 &  55.38 &  56.30 & 56.70 & 56.89 & 56.95 & 47.87 & 55.56 & 56.44 & 56.83 &  57.03 & 57.09 \\

 & DateAsTag & 42.03 & 49.47 &  50.38 & 50.81 &  51.03 & 51.09 & 43.11 & 50.32 & 51.23 & 51.63 &  51.85 & 51.92 \\
 & DateEmbedding & 50.09& 58.12 &  58.93 & 59.30 &  59.50 &  59.54 & 50.61 &58.41 & 59.25 & 59.63 &59.81 &   59.86 \\


%MSS-DPR         &  &  &  & &  &  & &  &   & &  &  \\
\midrule
\multirow{4}{*}{\textbf{ChroniclingQA}} & NoDate & 39.72 & 44.90 & 45.44 & 45.70 & 45.88 & 45.92 & 41.2 & 45.75 & 46.29 & 46.53 & 46.68 & 46.71 \\
 & DateAsToken & 39.72 & 44.90 & 45.44 & 45.70 & 45.88 & 45.92 & 41.2 & 45.75 & 46.29 & 46.53 & 46.68 & 46.71\\
 & DateAsTag & 40.21 & 45.00 & 45.51 & 45.76 & 45.95 & 46.00 & 41.2 & 45.41 & 45.98 & 46.29 & 46.43 & 46.48 \\
 & DateEmbedding & 44.35 & 49.78 & 50.29 & 50.61 & 50.77 & 50.82 & 44.83 & 49.52 & 50.09 & 50.38 & 50.57 & 50.60 \\
\bottomrule

\end{tabular}}
\caption{Results (MAP@\{1,5,10,20,50,100\}) for the ArchivalQA and ChroniclingQA explicit datasets across validation and test sets.}
\end{table}
\end{comment}





\begin{table}[ht]
\centering
\setlength\tabcolsep{5pt}
\resizebox{1\textwidth}{!}{  % Resize the table to fit the page width

\begin{tabular}{l|l|cccccc|cccccc} %|cccccc
\hline
\multirow{3}{*}{\textbf{Retriever}} & \multirow{3}{*}{\textbf{Mode}}& \multicolumn{12}{c}{\textbf{nDCG}} \\
\cline{3-14}
&   & \multicolumn{6}{c|}{\textbf{Val }} & \multicolumn{6}{c}{\textbf{Test}}  \\ %& \multicolumn{6}{c}{\textbf{WEBQ}}
 & &1 & 5 & 10 & 20 & 50 & 100 & 1 & 5 & 10 & 20 & 50 & 100  \\ %& Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100

\midrule
\multirow{4}{*}{\textbf{ArchivalQA}}
& NoDate  & 48.59 & 59.20 & 61.25 & 62.49 & 63.69 & 64.31
& 48.66& 59.38 & 61.25 & 62.61 & 63.84 &  64.43 \\

 & DateAsToken & 47.61& 58.48 & 60.71  &  62.17 &  63.35 & 63.95 
 & 47.89 & 58.64 & 60.76 & 62.17 &63.42 &  64.05\\

 & DateAsTag & 42.06 &  52.49 & 54.71 &  56.26&57.62  &58.31  
 &43.12  & 53.27 & 55.47 &  56.96 &58.32 &  59.04 \\
 
 & TempDPR & \textbf{50.12} & \textbf{61.25} & \textbf{63.22} & \textbf{64.55} & \textbf{65.73} & \textbf{66.24} 
 & \textbf{50.62} &\textbf{61.49} & \textbf{63.53} &\textbf{64.91} & \textbf{66.05} & \textbf{66.54} \\
%MSS-DPR         &  &  &  & &  &  & &  &   & &  &  \\


\midrule
\multirow{4}{*}{\textbf{ChroniclingQA}} 
& NoDate & 39.72 & 47.06 & 48.35 & 49.36 & 50.38 & 50.86 
& 41.2 & 47.54 & 48.87 & 49.74 & 50.68 & 50.97 \\

 & DateAsToken & 39.72 & 47.06 & 48.35 & 49.36 & 50.38 & 50.86 
 & 41.2 & 47.54 & 48.87 & 49.74 & 50.68 & 50.97 \\
 
 & DateAsTag & 40.21 & 47.00 & 48.24 & 49.16 & 50.31 & 50.82 
 & 41.2 & 47.03 & 48.41 & 49.55 & 50.39 & 50.93 \\
 
 & TempDPR & \textbf{44.35} & \textbf{51.79} & \textbf{53.03} & \textbf{54.23} & \textbf{55.24} & \textbf{55.75} 
 & \textbf{44.83} & \textbf{51.44} & \textbf{52.85} & \textbf{53.88} & \textbf{55.01} & \textbf{55.33} \\

\bottomrule
\end{tabular}}

\resizebox{1\textwidth}{!}{  % Resize the table to fit the page width
\begin{tabular}{l|l|cccccc|cccccc} %|cccccc
\hline
\multirow{3}{*}{\textbf{Retriever}} & \multirow{3}{*}{\textbf{Mode}}& \multicolumn{12}{c}{\textbf{MAP}} \\
\cline{3-14}
&  & \multicolumn{6}{c|}{\textbf{Val }} & \multicolumn{6}{c}{\textbf{Test}}  \\ %& \multicolumn{6}{c}{\textbf{WEBQ}}
 & &1 & 5 & 10 & 20 & 50 & 100 & 1 & 5 & 10 & 20 & 50 & 100  \\ %& Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100

\midrule
\multirow{4}{*}{\textbf{ArchivalQA}} 
& NoDate & 48.56 & 56.17 & 57.02 &57.36  & 57.56 & 57.62 
& 48.64 & 56.33 & 57.12 &57.49 & 57.69&  57.74\\

 & DateAsToken & 47.58 &  55.38 &  56.30 & 56.70 & 56.89 & 56.95 
 & 47.87 & 55.56 & 56.44 & 56.83 &  57.03 & 57.09 \\

 & DateAsTag & 42.03 & 49.47 &  50.38 & 50.81 &  51.03 & 51.09 
 & 43.11 & 50.32 & 51.23 & 51.63 &  51.85 & 51.92 \\
 
 & TempDPR & \textbf{50.09} & \textbf{58.12} &  \textbf{58.93} & \textbf{59.30} &  \textbf{59.50} &  \textbf{59.54} 
 & \textbf{50.61} &\textbf{58.41} & \textbf{59.25} & \textbf{59.63} &\textbf{59.81} &   \textbf{59.86} \\


%MSS-DPR         &  &  &  & &  &  & &  &   & &  &  \\
\midrule
\multirow{4}{*}{\textbf{ChroniclingQA}} 
& NoDate & 39.72 & 44.90 & 45.44 & 45.70 & 45.88 & 45.92 
& 41.2 & 45.75 & 46.29 & 46.53 & 46.68 & 46.71 \\

 & DateAsToken & 39.72 & 44.90 & 45.44 & 45.70 & 45.88 & 45.92 
 & 41.2 & 45.75 & 46.29 & 46.53 & 46.68 & 46.71\\
 
 & DateAsTag & 40.21 & 45.00 & 45.51 & 45.76 & 45.95 & 46.00 
 & 41.2 & 45.41 & 45.98 & 46.29 & 46.43 & 46.48 \\
 
 & TempDPR & \textbf{44.35} & \textbf{49.78} & \textbf{50.29} & \textbf{50.61} & \textbf{50.77} & \textbf{50.82} 
 & \textbf{44.83} & \textbf{49.52} & \textbf{50.09} & \textbf{50.38} & \textbf{50.57} & \textbf{50.60} \\
\bottomrule

\end{tabular}}
\caption{Results nDCG@\{1,5,10,20,50,100\} and MAP@\{1,5,10,20,50,100\} for the ArchivalQA and ChroniclingQA explicit datasets across validation and test sets.}
\label{tab:map_ndcg-explicit_dataset}
\end{table}






\begin{table}[ht]
\centering
\setlength\tabcolsep{5pt}
\resizebox{1\textwidth}{!}{  % Resize the table to fit the page width

\begin{tabular}{l|l|cccccc|cccccc} %|cccccc
\hline
\multirow{2}{*}{\textbf{Dataset}}& \multirow{2}{*}{\textbf{Mode}}  & \multicolumn{6}{c|}{\textbf{Val }} & \multicolumn{6}{c}{\textbf{Test}}  \\ %& \multicolumn{6}{c}{\textbf{WEBQ}}
  & &Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100 & Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100  \\ %& Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100

\midrule
\multirow{3}{*}{\textbf{ArchivalQA}} & NoDate & 44.39 & 67.35  & 74.97 & 81.23 & 87.44 & 90.98 & 43.83 & 66.61 & 74.23 & 80.55 & 87.04 &90.84 \\

 & DateAsToken  &  65.19 & 85.10 &  89.85 & 93.26&  96.20 & 97.47 & 65.12 &85.13 & 89.92& 93.28 & 96.15 & 97.56 \\

 %& DateAsTag &  & &  & &  & & &  &  & &  &  \\
 
 & TempDPR &  \textbf{78.93} & \textbf{93.86}& \textbf{96.33}  & \textbf{97.76} & \textbf{98.81} & \textbf{99.21}& \textbf{79.45} & \textbf{93.90} & \textbf{96.27} & \textbf{97.68}&  \textbf{98.74} & \textbf{99.20} \\
%MSS-DPR         &  &  &  & &  &  & &  &   & &  &  \\


\midrule
\multirow{3}{*}{\textbf{ChroniclingQA}} & NoDate & 49.36 &65.02 & 70.44 &75.19 & 80.58 &83.81 & 49.35& 64.89 & 70.71 & 75.40& 80.55 & 83.88 \\
 & DateAsToken &47.08  &63.60 & 69.65 &74.98 & 80.52 & 84.07 &46.54  &63.40  &69.60 &74.84 &80.71 & 84.21 \\
 %& DateAsTag &  & &  & &  & & &  &  & &  &  \\
 & TempDPR &\textbf{68.03}  &\textbf{86.22} &\textbf{92.33} &\textbf{96.56} & \textbf{98.79} &\textbf{99.22} & \textbf{68.07}& \textbf{86.52} & \textbf{92.17} &\textbf{96.25} &\textbf{98.67}  &\textbf{99.18}  \\

\bottomrule
\end{tabular}}
\setlength\tabcolsep{10.5pt}
\resizebox{1\textwidth}{!}{  % Resize the table to fit the page width

\begin{tabular}{l|l|ccc|ccc|ccc|ccc} %|cccccc
\hline
\multirow{3}{*}{\textbf{Dataset}}& \multirow{3}{*}{\textbf{Mode}}  & \multicolumn{6}{c|}{\textbf{Val }} & \multicolumn{6}{c}{\textbf{Test}}  \\ 

 & & \multicolumn{3}{c}{\textbf{nDCG}} & \multicolumn{3}{c|}{\textbf{MAP}} & \multicolumn{3}{c}{\textbf{nDCG}} & \multicolumn{3}{c}{\textbf{MAP}}  \\ 
 & &1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10  \\ 


\midrule
\multirow{3}{*}{\textbf{ArchivalQA}} & NoDate & 30.59 & 39.96 &42.28  & 30.57 & 37.20 & 38.15 & 30.59 & 39.96 & 42.28 & 30.57 &37.20  & 38.15\\

 & DateAsToken & 49.61 & 60.28 & 62.41 & 49.58 & 57.21 &58.10 & 49.76 & 60.49 & 62.67 & 49.73 & 57.39 & 58.29 \\ 

 %& DateAsTag &  & &  & &  & & &  &  & &  &  \\
 
 & TempDPR &  \textbf{72.19} & \textbf{81.86} &  \textbf{82.97} & \textbf{72.13} & \textbf{79.23} & \textbf{79.70} & \textbf{72.76} & \textbf{82.27} &\textbf{83.34}  & \textbf{72.71} & \textbf{79.68} &   \textbf{80.13}\\

\midrule
\multirow{3}{*}{\textbf{ChroniclingQA}} & NoDate &42.22  &48.95 &50.17  &42.22 &47.06  &47.56 &42.46 &49.20  &50.44  &42.46 & 47.29 &47.81   \\
 & DateAsToken & 39.23 &46.46  & 47.93 &39.23 &44.38  & 44.99& 39.02 & 46.48 & 47.91 & 39.02 & 44.36 &44.96  \\
% & DateAsTag &  & &  & &  & & &  &  & &  &  \\
 & TempDPR &\textbf{62.40}  &\textbf{73.37} & \textbf{75.74} &\textbf{62.40} & \textbf{70.23} & \textbf{71.21} & \textbf{62.41} & \textbf{73.54} &\textbf{75.80}  &\textbf{62.41} &\textbf{70.38}  & \textbf{71.32} \\

\bottomrule
\end{tabular}}
\caption{ Top-\{1,5,10,20,50,100\}, nDCG@\{1,5,10,20,50,100\} and MAP@\{1,5,10,20,50,100\} for the ArchivalQA and ChroniclingQA across FULL validation and test sets.}
\label{tab:oracle_result}
\end{table}



\begin{comment}
    
\begin{table}[ht]
\centering
\resizebox{1\textwidth}{!}{  % Resize the table to fit the page width

\begin{tabular}{l|l|ccc|ccc|ccc|ccc} %|cccccc
\hline
\multirow{3}{*}{\textbf{Retriever}}& \multirow{3}{*}{\textbf{Mode}}  & \multicolumn{6}{c|}{\textbf{Val }} & \multicolumn{6}{c}{\textbf{Test}}  \\ 

 & & \multicolumn{3}{c}{\textbf{NDCG}} & \multicolumn{3}{c|}{\textbf{MAP}} & \multicolumn{3}{c}{\textbf{NDCG}} & \multicolumn{3}{c}{\textbf{MAP}}  \\ 
 & &1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10  \\ 


\midrule
\multirow{3}{*}{\textbf{ArchivalQA}} & NoDate & 30.59 & 39.96 &42.28  & 30.57 & 37.20 & 38.15 & 30.59 & 39.96 & 42.28 & 30.57 &37.20  & 38.15\\

 & DateAsToken & 49.61 & 60.28 & 62.41 & 49.58 & 57.21 &58.10 & 49.76 & 60.49 & 62.67 & 49.73 & 57.39 & 58.29 \\ 

 %& DateAsTag &  & &  & &  & & &  &  & &  &  \\
 
 & DateEmbedding &  72.19 & 81.86 &  82.97 & 72.13 & 79.23 & 79.70 & 72.76 & 82.27 &83.34  & 72.71 & 79.68 &   80.13\\

\midrule
\multirow{3}{*}{\textbf{ChroniclingQA}} & NoDate &42.22  &48.95 &50.17  &42.22 &47.06  &47.56 &42.46 &49.20  &50.44  &42.46 & 47.29 &47.81   \\
 & DateAsToken & 39.23 &46.46  & 47.93 &39.23 &44.38  & 44.99& 39.02 & 46.48 & 47.91 & 39.02 & 44.36 &44.96  \\
% & DateAsTag &  & &  & &  & & &  &  & &  &  \\
 & DateEmbedding &62.40  &73.37 & 75.74 &62.40 & 70.23 & 71.21 & 62.41 & 73.54 &75.80  &62.41 &70.38  & 71.32 \\

\bottomrule
\end{tabular}}
\caption{Oracle NDCG and MAP}
\end{table}

\end{comment}

\begin{comment}
    
\begin{table}[ht]
\centering
\resizebox{1\textwidth}{!}{  % Resize the table to fit the page width

\begin{tabular}{l|l|cccccc|cccccc} %|cccccc
\hline
\multirow{2}{*}{\textbf{Retriever}}& \multirow{2}{*}{\textbf{Mode}}  & \multicolumn{6}{c|}{\textbf{Val }} & \multicolumn{6}{c}{\textbf{Test}}  \\ %& \multicolumn{6}{c}{\textbf{WEBQ}}
 & &1 & 5 & 10 & 20 & 50 & 100 & 1 & 5 & 10 & 20 & 50 & 100  \\ %& Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100

\midrule
\multirow{4}{*}{\textbf{ArchivalQA}} & NoDate & 0.23288 & 0.30124 & 0.32349 & 0.33918 & 0.3592 & 0.36889 & 0.22234 & 0.2943 & 0.3146 & 0.33021 & 0.34961 & 0.3595 \\
 & DateAsToken & 0.21235 & 0.28778 & 0.31112 & 0.3328 & 0.35346 & 0.3659 & 0.20179 & 0.27624 & 0.30155 & 0.32314 & 0.34498 & 0.35539 \\
 & DateAsTag & 0.44038 & 0.63315 & 0.69679 & 0.75271 & 0.81992 & 0.86137 & 0.43229 & 0.62938 & 0.69478 & 0.75504 & 0.82269 & 0.86515 \\
 & DateEmbedding & 0.50089 & 0.70578 & 0.76648 & 0.81884 & 0.87795 & 0.90894 & 0.5061 & 0.70699 & 0.76982 & 0.8243 & 0.88179 & 0.9116 \\


%MSS-DPR         &  &  &  & &  &  & &  &   & &  &  \\
\midrule
\multirow{4}{*}{\textbf{ChroniclingQA}} & NoDate & 0.39724 & 0.53534 & 0.57514 & 0.61576 & 0.66613 & 0.69537 & 0.412 & 0.52881 & 0.57064 & 0.60458 & 0.65193 & 0.6693 \\
 & DateAsToken & 0.39724 & 0.53534 & 0.57514 & 0.61576 & 0.66613 & 0.69537 & 0.412 & 0.52881 & 0.57064 & 0.60458 & 0.65193 & 0.6693 \\
 & DateAsTag & 0.40211 & 0.53046 & 0.56864 & 0.6052 & 0.66288 & 0.69374 & 0.412 & 0.51855 & 0.56117 & 0.60616 & 0.64878 & 0.68114 \\
 & DateEmbedding & 0.44354 & 0.57758 & 0.61576 & 0.66369 & 0.71487 & 0.74574 & 0.4483 & 0.57222 & 0.61642 & 0.65667 & 0.71271 & 0.73244 \\

\bottomrule
\end{tabular}}
\caption{Recall}
\end{table}
\end{comment}




==> tables/_backup_old_tables.tex <==
\begin{table}[ht]
\centering
\resizebox{1\textwidth}{!}{  % Resize the table to fit the page width

\begin{tabular}{l|l|cccccc|cccccc} %|cccccc
\hline
\multirow{2}{*}{\textbf{Retriever}}& \multirow{2}{*}{\textbf{Mode}}  & \multicolumn{6}{c|}{\textbf{Val }} & \multicolumn{6}{c}{\textbf{ Test }}  \\ %& \multicolumn{6}{c}{\textbf{WEBQ}}
 & &Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100 & Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100  \\ %& Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100

\midrule


\multirow{4}{*}{\textbf{ArchivalQA}} & NoDate 
  & $63.09 \pm 0.76$  & $82.42 \pm 0.29$  & $87.47 \pm 0.11$  & $90.97 \pm 0.15$  & $94.40 \pm 0.21$  & $96.14 \pm 0.03$
  & $62.98 \pm 0.55$  & $82.50 \pm 0.33$  & $87.17 \pm 0.45$  & $90.97 \pm 0.27$  & $94.64 \pm 0.23$  & $96.15 \pm 0.16$   \\
  
  & DateAsToken   
  & $63.51 \pm 0.32$  & $83.41 \pm 0.28$  & $88.52 \pm 0.08$  & $91.97 \pm 0.08$  & $94.92 \pm 0.05$  & $96.52 \pm 0.02$  
  & $63.44 \pm 0.29$  & $83.23 \pm 0.05$  & $88.35 \pm 0.10$  & $91.72 \pm 0.03$  & $94.94 \pm 0.23$  & $96.72 \pm 0.08$\\

  & DateAsTag 
  & $57.94 \pm 0.71$  & $78.78 \pm 0.61$  & $84.28 \pm 0.41$  & $88.48 \pm 0.48$  & $92.43 \pm 0.26$  & $94.64 \pm 0.13$ 
  & $58.37 \pm 0.70$  & $78.43 \pm 0.84$  & $83.93 \pm 0.45$  & $88.21 \pm 0.41$  & $92.77 \pm 0.25$  & $94.93 \pm 0.10$  \\
  
  & DateEmbedding   
  & $64.80 \pm 0.34$  & $84.95 \pm 0.32$  & $89.35 \pm 0.09$  & $92.63 \pm 0.06$  & $95.41 \pm 0.12$  & $96.73 \pm 0.03$  
    & $65.10 \pm 0.86$  & $84.78 \pm 0.46$  & $89.42 \pm 0.36$  & $92.84 \pm 0.35$  & $95.77 \pm 0.23$  & $97.13 \pm 0.13$ \\
\bottomrule

\multirow{4}{*}{\textbf{ChroniclingQA}} & NoDate 
  & $44.97 \pm 0.24$  & $61.14 \pm 0.16$  & $67.86 \pm 0.16$  & $73.32 \pm 0.21$  & $79.12 \pm 0.10$  & $83.53 \pm 0.15$ 
    & $45.70 \pm 0.46$  & $60.47 \pm 0.25$  & $67.40 \pm 0.14$  & $72.20 \pm 0.18$  & $78.69 \pm 0.13$  & $82.26 \pm 0.09$ \\
  
  & DateAsToken 
  & $44.81 \pm 0.04$  & $61.28 \pm 0.28$  & $67.62 \pm 0.16$  & $73.60 \pm 0.13$  & $79.12 \pm 0.25$  & $83.17 \pm 0.07$
    & $45.81 \pm 0.09$  & $60.79 \pm 0.19$  & $66.58 \pm 0.20$  & $72.09 \pm 0.15$  & $78.82 \pm 0.07$  & $82.10 \pm 0.22$  \\
  
  & DateAsTag 
  & $45.00 \pm 0.17$  & $61.48 \pm 0.31$  & $67.62 \pm 0.19$  & $72.97 \pm 0.07$  & $79.14 \pm 0.18$  & $82.99 \pm 0.18$
    & $45.75 \pm 0.48$  & $60.77 \pm 0.49$  & $66.77 \pm 0.22$  & $72.44 \pm 0.32$  & $78.72 \pm 0.18$  & $81.89 \pm 0.21$  \\
  
  & DateEmbedding  
  & $50.22 \pm 0.19$  & $64.88 \pm 0.23$  & $71.16 \pm 0.30$  & $77.90 \pm 0.21$  & $83.05 \pm 0.11$  & $86.22 \pm 0.29$
    & $50.10 \pm 0.10$  & $66.01 \pm 0.17$  & $71.85 \pm 0.39$  & $77.19 \pm 0.11$  & $82.81 \pm 0.25$  & $86.52 \pm 0.10$  \\
\bottomrule
\end{tabular}}
\caption{Top-\{1,5,10,20,50,100\} retrieval accuracy for ArchivalQA and ChroniclingQA explicit datasets, evaluated on both validation and test sets. The results measure the percentage of top retrieved passages that contain the correct answer across different temporal retrieval models, including the baseline Vanilla, Date as Token, Date as Tag, and Date Embedding approaches.}
\end{table}



    
\begin{table}[ht]
\centering
\resizebox{1\textwidth}{!}{  % Resize the table to fit the page width

\begin{tabular}{l|l|cccccc|cccccc} %|cccccc
\hline
\multirow{2}{*}{\textbf{Retriever}}& \multirow{2}{*}{\textbf{Mode}}  & \multicolumn{6}{c|}{\textbf{Val }} & \multicolumn{6}{c}{\textbf{Test}}  \\ %& \multicolumn{6}{c}{\textbf{WEBQ}}
 & &1 & 5 & 10 & 20 & 50 & 100 & 1 & 5 & 10 & 20 & 50 & 100  \\ %& Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100

\midrule
\multirow{4}{*}{\textbf{ArchivalQA}} & NoDate  & 48.59 & 59.20 & 61.25 & 62.49 & 63.69 & 64.31 & 48.66& 59.38 & 61.25 & 62.61 & 63.84 &  64.43 \\



 & DateAsToken & 47.61& 58.48 & 60.71  &  62.17 &  63.35 & 63.95 & 47.89 & 58.64 & 60.76 & 62.17&63.42 &  64.05\\



 & DateAsTag & 42.06 &  52.49 & 54.71 &  56.26&57.62  &58.31  &43.12  & 53.27 & 55.47 &  56.96&58.32 &  59.04 \\
 


 & DateEmbedding & 50.12 & 61.25 & 63.22 & 64.55 & 65.73 & 66.24 & 50.62 &61.49 & 63.53 &64.91 & 66.05 & 66.54 \\
%MSS-DPR         &  &  &  & &  &  & &  &   & &  &  \\


\midrule
\multirow{4}{*}{\textbf{ChroniclingQA}} & NoDate & 39.72 & 47.06 & 48.35 & 49.36 & 50.38 & 50.86 & 41.2 & 47.54 & 48.87 & 49.74 & 50.68 & 50.97 \\
 & DateAsToken & 39.72 & 47.06 & 48.35 & 49.36 & 50.38 & 50.86 & 41.2 & 47.54 & 48.87 & 49.74 & 50.68 & 50.97 \\
 & DateAsTag & 40.21 & 47.00 & 48.24 & 49.16 & 50.31 & 50.82 & 41.2 & 47.03 & 48.41 & 49.55 & 50.39 & 50.93 \\
 & DateEmbedding & 44.35 & 51.79 & 53.03 & 54.23 & 55.24 & 55.75 & 44.83 & 51.44 & 52.85 & 53.88 & 55.01 & 55.33 \\

\bottomrule
\end{tabular}}
\caption{Results (NDCG@\{1,5,10,20,50,100\}) for the ArchivalQA and ChroniclingQA explicit datasets across validation and test sets.}
\end{table}


\begin{table}[ht]
\centering
\resizebox{1\textwidth}{!}{  % Resize the table to fit the page width

\begin{tabular}{l|l|cccccc|cccccc} %|cccccc
\hline
\multirow{2}{*}{\textbf{Retriever}}& \multirow{2}{*}{\textbf{Mode}}  & \multicolumn{6}{c|}{\textbf{Val }} & \multicolumn{6}{c}{\textbf{Test}}  \\ %& \multicolumn{6}{c}{\textbf{WEBQ}}
 & &1 & 5 & 10 & 20 & 50 & 100 & 1 & 5 & 10 & 20 & 50 & 100  \\ %& Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100

\midrule
\multirow{4}{*}{\textbf{ArchivalQA}} & NoDate & 48.56 & 56.17 & 57.02 &57.36  & 57.56 & 57.62 & 48.64 & 56.33 & 57.12 &57.49 & 57.69&  57.74\\

 & DateAsToken & 47.58 &  55.38 &  56.30 & 56.70 & 56.89 & 56.95 & 47.87 & 55.56 & 56.44 & 56.83 &  57.03 & 57.09 \\

 & DateAsTag & 42.03 & 49.47 &  50.38 & 50.81 &  51.03 & 51.09 & 43.11 & 50.32 & 51.23 & 51.63 &  51.85 & 51.92 \\
 & DateEmbedding & 50.09& 58.12 &  58.93 & 59.30 &  59.50 &  59.54 & 50.61 &58.41 & 59.25 & 59.63 &59.81 &   59.86 \\



%MSS-DPR         &  &  &  & &  &  & &  &   & &  &  \\
\midrule
\multirow{4}{*}{\textbf{ChroniclingQA}} & NoDate & 39.72 & 44.90 & 45.44 & 45.70 & 45.88 & 45.92 & 41.2 & 45.75 & 46.29 & 46.53 & 46.68 & 46.71 \\
 & DateAsToken & 39.72 & 44.90 & 45.44 & 45.70 & 45.88 & 45.92 & 41.2 & 45.75 & 46.29 & 46.53 & 46.68 & 46.71\\
 & DateAsTag & 40.21 & 45.00 & 45.51 & 45.76 & 45.95 & 46.00 & 41.2 & 45.41 & 45.98 & 46.29 & 46.43 & 46.48 \\
 & DateEmbedding & 44.35 & 49.78 & 50.29 & 50.61 & 50.77 & 50.82 & 44.83 & 49.52 & 50.09 & 50.38 & 50.57 & 50.60 \\
\bottomrule

\end{tabular}}
\caption{Results (MAP@\{1,5,10,20,50,100\}) for the ArchivalQA and ChroniclingQA explicit datasets across validation and test sets.}
\end{table}




\begin{table}[ht]
\centering
\resizebox{1\textwidth}{!}{  % Resize the table to fit the page width

\begin{tabular}{l|l|cccccc|cccccc} %|cccccc
\hline
\multirow{2}{*}{\textbf{Retriever}}& \multirow{2}{*}{\textbf{Mode}}  & \multicolumn{6}{c|}{\textbf{Val }} & \multicolumn{6}{c}{\textbf{Test}}  \\ %& \multicolumn{6}{c}{\textbf{WEBQ}}
 & &1 & 5 & 10 & 20 & 50 & 100 & 1 & 5 & 10 & 20 & 50 & 100  \\ %& Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100

\midrule
\multirow{3}{*}{\textbf{ArchivalQA}} & NoDate & 44.39 & 67.35  & 74.97 & 81.23 & 87.44 & 90.98 & 43.83 & 66.61 & 74.23 & 80.55 & 87.04 &90.84 \\



 & DateAsToken  &  65.19 & 85.10 &  89.85 & 93.26&  96.20 & 97.47 & 65.12 &85.13 & 89.92& 93.28 & 96.15 & 97.56 \\

 %& DateAsTag &  & &  & &  & & &  &  & &  &  \\
 


 & DateEmbedding &  78.93 & 93.86 & 96.33  & 97.76 & 98.81 & 99.21& 79.45 & 93.90 & 96.27 & 97.68&  98.74 & 99.20 \\
%MSS-DPR         &  &  &  & &  &  & &  &   & &  &  \\




\midrule
\multirow{3}{*}{\textbf{ChroniclingQA}} & NoDate & 49.36 &65.02 & 70.44 &75.19 & 80.58 &83.81 & 49.35& 64.89 & 70.71 & 75.40& 80.55 & 83.88 \\
 & DateAsToken &47.08  &63.60 & 69.65 &74.98 & 80.52 & 84.07 &46.54  &63.40  &69.60 &74.84 &80.71 & 84.21 \\
 %& DateAsTag &  & &  & &  & & &  &  & &  &  \\
 & DateEmbedding &68.03  &86.22 &92.33 &96.56 & 98.79 &99.22 & 68.07& 86.52 & 92.17 &96.25 &98.67  &99.18  \\

\bottomrule
\end{tabular}}
\caption{Oracle Top}
\end{table}




\begin{table}[ht]
\centering
\resizebox{1\textwidth}{!}{  % Resize the table to fit the page width

\begin{tabular}{l|l|ccc|ccc|ccc|ccc} %|cccccc
\hline
\multirow{3}{*}{\textbf{Retriever}}& \multirow{3}{*}{\textbf{Mode}}  & \multicolumn{6}{c|}{\textbf{Val }} & \multicolumn{6}{c}{\textbf{Test}}  \\ 

 & & \multicolumn{3}{c}{\textbf{NDCG}} & \multicolumn{3}{c|}{\textbf{MAP}} & \multicolumn{3}{c}{\textbf{NDCG}} & \multicolumn{3}{c}{\textbf{MAP}}  \\ 
 & &1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10  \\ 


\midrule
\multirow{3}{*}{\textbf{ArchivalQA}} & NoDate & 30.59 & 39.96 &42.28  & 30.57 & 37.20 & 38.15 & 30.59 & 39.96 & 42.28 & 30.57 &37.20  & 38.15\\






 & DateAsToken & 49.61 & 60.28 & 62.41 & 49.58 & 57.21 &58.10 & 49.76 & 60.49 & 62.67 & 49.73 & 57.39 & 58.29 \\ 



 %& DateAsTag &  & &  & &  & & &  &  & &  &  \\
 


 & DateEmbedding &  72.19 & 81.86 &  82.97 & 72.13 & 79.23 & 79.70 & 72.76 & 82.27 &83.34  & 72.71 & 79.68 &   80.13\\

\midrule
\multirow{3}{*}{\textbf{ChroniclingQA}} & NoDate &42.22  &48.95 &50.17  &42.22 &47.06  &47.56 &42.46 &49.20  &50.44  &42.46 & 47.29 &47.81   \\
 & DateAsToken & 39.23 &46.46  & 47.93 &39.23 &44.38  & 44.99& 39.02 & 46.48 & 47.91 & 39.02 & 44.36 &44.96  \\
% & DateAsTag &  & &  & &  & & &  &  & &  &  \\
 & DateEmbedding &62.40  &73.37 & 75.74 &62.40 & 70.23 & 71.21 & 62.41 & 73.54 &75.80  &62.41 &70.38  & 71.32 \\

\bottomrule
\end{tabular}}
\caption{Oracle NDCG and MAP}
\end{table}



\begin{comment}
    
\begin{table}[ht]
\centering
\resizebox{1\textwidth}{!}{  % Resize the table to fit the page width

\begin{tabular}{l|l|cccccc|cccccc} %|cccccc
\hline
\multirow{2}{*}{\textbf{Retriever}}& \multirow{2}{*}{\textbf{Mode}}  & \multicolumn{6}{c|}{\textbf{Val }} & \multicolumn{6}{c}{\textbf{Test}}  \\ %& \multicolumn{6}{c}{\textbf{WEBQ}}
 & &1 & 5 & 10 & 20 & 50 & 100 & 1 & 5 & 10 & 20 & 50 & 100  \\ %& Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100

\midrule
\multirow{4}{*}{\textbf{ArchivalQA}} & NoDate & 0.23288 & 0.30124 & 0.32349 & 0.33918 & 0.3592 & 0.36889 & 0.22234 & 0.2943 & 0.3146 & 0.33021 & 0.34961 & 0.3595 \\
 & DateAsToken & 0.21235 & 0.28778 & 0.31112 & 0.3328 & 0.35346 & 0.3659 & 0.20179 & 0.27624 & 0.30155 & 0.32314 & 0.34498 & 0.35539 \\
 & DateAsTag & 0.44038 & 0.63315 & 0.69679 & 0.75271 & 0.81992 & 0.86137 & 0.43229 & 0.62938 & 0.69478 & 0.75504 & 0.82269 & 0.86515 \\
 & DateEmbedding & 0.50089 & 0.70578 & 0.76648 & 0.81884 & 0.87795 & 0.90894 & 0.5061 & 0.70699 & 0.76982 & 0.8243 & 0.88179 & 0.9116 \\


%MSS-DPR         &  &  &  & &  &  & &  &   & &  &  \\
\midrule
\multirow{4}{*}{\textbf{ChroniclingQA}} & NoDate & 0.39724 & 0.53534 & 0.57514 & 0.61576 & 0.66613 & 0.69537 & 0.412 & 0.52881 & 0.57064 & 0.60458 & 0.65193 & 0.6693 \\
 & DateAsToken & 0.39724 & 0.53534 & 0.57514 & 0.61576 & 0.66613 & 0.69537 & 0.412 & 0.52881 & 0.57064 & 0.60458 & 0.65193 & 0.6693 \\
 & DateAsTag & 0.40211 & 0.53046 & 0.56864 & 0.6052 & 0.66288 & 0.69374 & 0.412 & 0.51855 & 0.56117 & 0.60616 & 0.64878 & 0.68114 \\
 & DateEmbedding & 0.44354 & 0.57758 & 0.61576 & 0.66369 & 0.71487 & 0.74574 & 0.4483 & 0.57222 & 0.61642 & 0.65667 & 0.71271 & 0.73244 \\

\bottomrule
\end{tabular}}
\caption{Recall}
\end{table}
\end{comment}




==> tables/implicit_ndcg_result.tex <==
\begin{table*}[ht]
\centering
\caption{Results for nDCG@\{1,5,10,20,50,100\} for the implicit questions from \textit{ArchivalQA} datasets, across validation and test sets.}
\setlength\tabcolsep{5pt}
\resizebox{\textwidth}{!}{  % Resize the table to fit the page width
\begin{tabular}{l|l|cccccc|cccccc}  
\hline
\multirow{3}{*}{\textbf{Retriever}} & \multirow{3}{*}{\textbf{Mode}} 
& \multicolumn{12}{c}{\textbf{nDCG}} \\ 
\cline{3-14}
 &  & \multicolumn{6}{c|}{\textbf{Validation}} & \multicolumn{6}{c}{\textbf{Test}} \\ 
\cline{3-14}
 &  & @1 & @5 & @10 & @20 & @50 & @100 
 & @1 & @5 & @10 & @20 & @50 & @100 \\

\midrule
\multirow{4}{*}{\textbf{ArchivalQA}} 
 & \Vanilla 
 & 28.30 & 36.98 & 39.14 & 40.89 & 42.57  & 43.78
 & 28.25 & 34.54 & 35.42 & 35.91 & 36.18 & 36.29\\ 
 
 & BiTimeBERT 
 & 14.90 & 22.01 & 24.66 & 26.18 & 28.16 & 29.29
 & 14.90 & 19.96 & 21.05 & 21.46 & 21.78 & 21.88\\ 

 & TS Retriever 
 & 26.80 & 36.00 & 38.76 & 40.44 & 42.01 & 43.23
 & 26.75 & 33.27 & 34.40 & 34.87 & 35.13 & 35.24\\ 

 & \DateTag 
 & 27.0 & 35.08 & 37.11 & 38.78 & 40.64 & 41.53
 & 25.6 & 34.56 & 36.82 & 38.05 & 39.76 & 40.73 \\ 

 & \DateToken 
 & 27.9 & 36.53 & 38.68 & 40.38 & 42.00 & 43.16
 & 28.3 & 36.30 & 38.56 & 40.05 & 41.55 & 42.56 \\ 

 & \TempDPR$_{FS}$
 & 29.60 & 38.59 & 40.58 & 42.42 & 44.16  & 45.09
 & 30.30 & 38.69 & 40.89 & 42.28 & 43.92 & 44.94\\ 

 & \TempDPR$_{VS}$
 & 30.30  & 39.25 & 41.40 & 42.95 & 44.61 & 45.59
 & 29.60 & 38.82 & 40.72 & 42.27 & 43.68 & 44.63\\ 

 & \TempDPR$_{EWI}$
 & 28.80 & 36.92 & 39.10 & 40.51 & 42.34 & 43.33
 & 26.40 & 35.32 & 37.12 & 38.60 & 40.32 & 41.36 \\ 

\bottomrule
\end{tabular}
}
\label{tab:map_ndcg-implict_dataset}
\end{table*}


==> tables/oracle_top_ndcg_result.tex <==
\begin{table*}[ht]
\centering
\caption{ Oracle results
%: Top-\{1,5,10,20,50,100\}, nDCG@\{1,5,10,20,50,100\} and MAP@\{1,5,10,20,50,100\} 
%for the \textit{ArchivalQA} and \textit{ChroniclingAmericaQA} 
across FULL validation and test sets of the \textit{ArchivalQA} and \textit{ChroniclingAmericaQA}.}
\setlength\tabcolsep{5pt}
\resizebox{0.7\textwidth}{!}{  % Resize the table to fit the page width

\begin{tabular}{l|l|cccccc|cccccc} %|cccccc
\hline
\multirow{2}{*}{\textbf{Dataset}}& \multirow{2}{*}{\textbf{Mode}}  & \multicolumn{6}{c|}{\textbf{Val }} & \multicolumn{6}{c}{\textbf{Test}}  \\ %& \multicolumn{6}{c}{\textbf{WEBQ}}
  & &Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100 & Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100  \\ %& Top-1 & Top-5 & Top-10 & Top-20 & Top-50 & Top-100

\midrule
\multirow{3}{*}{\textbf{ArchivalQA}} & \Vanilla & 44.39 & 67.35  & 74.97 & 81.23 & 87.44 & 90.98 & 43.83 & 66.61 & 74.23 & 80.55 & 87.04 &90.84 \\

 & \DateToken  &  65.19 & 85.10 &  89.85 & 93.26&  96.20 & 97.47 & 65.12 &85.13 & 89.92& 93.28 & 96.15 & 97.56 \\

 %& DateAsTag &  & &  & &  & & &  &  & &  &  \\
 
 & \TempDPR$_{\oplus}$  &  \textbf{78.93} & \textbf{93.86}& \textbf{96.33}  & \textbf{97.76} & \textbf{98.81} & \textbf{99.21}& \textbf{79.45} & \textbf{93.90} & \textbf{96.27} & \textbf{97.68}&  \textbf{98.74} & \textbf{99.20} \\
%MSS-DPR         &  &  &  & &  &  & &  &   & &  &  \\


\midrule
\multirow{3}{*}{\textbf{ChroniclingQA}} & \Vanilla & 49.36 &65.02 & 70.44 &75.19 & 80.58 &83.81 & 49.35& 64.89 & 70.71 & 75.40& 80.55 & 83.88 \\
 & \DateToken &47.08  &63.60 & 69.65 &74.98 & 80.52 & 84.07 &46.54  &63.40  &69.60 &74.84 &80.71 & 84.21 \\
 %& DateAsTag &  & &  & &  & & &  &  & &  &  \\
 & \TempDPR$_{\oplus}$  &\textbf{68.03}  &\textbf{86.22} &\textbf{92.33} &\textbf{96.56} & \textbf{98.79} &\textbf{99.22} & \textbf{68.07}& \textbf{86.52} & \textbf{92.17} &\textbf{96.25} &\textbf{98.67}  &\textbf{99.18}  \\

\bottomrule
\end{tabular}}
\setlength\tabcolsep{10.5pt}
\resizebox{0.7\textwidth}{!}{  % Resize the table to fit the page width

\begin{tabular}{l|l|ccc|ccc|ccc|ccc} %|cccccc
\hline
\multirow{3}{*}{\textbf{Dataset}}& \multirow{3}{*}{\textbf{Mode}}  & \multicolumn{6}{c|}{\textbf{Val }} & \multicolumn{6}{c}{\textbf{Test}}  \\ 

 & & \multicolumn{3}{c}{\textbf{nDCG}} & \multicolumn{3}{c|}{\textbf{MAP}} & \multicolumn{3}{c}{\textbf{nDCG}} & \multicolumn{3}{c}{\textbf{MAP}}  \\ 
 & &1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10  \\ 


\midrule
\multirow{3}{*}{\textbf{ArchivalQA}} & \Vanilla & 30.59 & 39.96 &42.28  & 30.57 & 37.20 & 38.15 & 30.59 & 39.96 & 42.28 & 30.57 &37.20  & 38.15\\

 & \DateToken & 49.61 & 60.28 & 62.41 & 49.58 & 57.21 &58.10 & 49.76 & 60.49 & 62.67 & 49.73 & 57.39 & 58.29 \\ 

 %& DateAsTag &  & &  & &  & & &  &  & &  &  \\
 
 & \TempDPR$_{\oplus}$  &  \textbf{72.19} & \textbf{81.86} &  \textbf{82.97} & \textbf{72.13} & \textbf{79.23} & \textbf{79.70} & \textbf{72.76} & \textbf{82.27} &\textbf{83.34}  & \textbf{72.71} & \textbf{79.68} &   \textbf{80.13}\\

\midrule
\multirow{3}{*}{\textbf{ChroniclingQA}} & \Vanilla &42.22  &48.95 &50.17  &42.22 &47.06  &47.56 &42.46 &49.20  &50.44  &42.46 & 47.29 &47.81   \\
 & \DateToken & 39.23 &46.46  & 47.93 &39.23 &44.38  & 44.99& 39.02 & 46.48 & 47.91 & 39.02 & 44.36 &44.96  \\
% & DateAsTag &  & &  & &  & & &  &  & &  &  \\
 & \TempDPR$_{\oplus}$  &\textbf{62.40}  &\textbf{73.37} & \textbf{75.74} &\textbf{62.40} & \textbf{70.23} & \textbf{71.21} & \textbf{62.41} & \textbf{73.54} &\textbf{75.80}  &\textbf{62.41} &\textbf{70.38}  & \textbf{71.32} \\

\bottomrule
\end{tabular}}

\label{tab:oracle_result}
\end{table*}
